Recovering the colour-dependent albedo of exoplanets with high-resolution spectroscopy: from ESPRESSO to the ELT

The characterization of planetary atmospheres is a daunting task, pushing current observing facilities to their limits. The next generation of high-resolution spectrographs mounted on large telescopes -- such as ESPRESSO@VLT and HIRES@ELT -- will allow us to probe and characterize exoplanetary atmospheres in greater detail than possible to this point. We present a method that permits the recovery of the colour-dependent reflectivity of exoplanets from high-resolution spectroscopic observations. Determining the wavelength-dependent albedo will provide insight into the chemical properties and weather of the exoplanet atmospheres. For this work, we simulated ESPRESSO@VLT and HIRES@ELT high-resolution observations of known planetary systems with several albedo configurations. We demonstrate how the cross correlation technique applied to theses simulated observations can be used to successfully recover the geometric albedo of exoplanets over a range of wavelengths. In all cases, we were able to recover the wavelength dependent albedo of the simulated exoplanets and distinguish between several atmospheric models representing different atmospheric configurations. In brief, we demonstrate that the cross correlation technique allows for the recovery of exoplanetary albedo functions from optical observations with the next generation of high-resolution spectrographs that will be mounted on large telescopes with reasonable exposure times. Its recovery will permit the characterization of exoplanetary atmospheres in terms of composition and dynamics and consolidates the cross correlation technique as a powerful tool for exoplanet characterization.

==> figures/tex_figure_espresso_hr_51_Peg_b_4days_A_g-0.2.tex <==
\begin{subfigure}[t]{0.5\hsize}
	\includegraphics[width=\hsize]{./figures/{recovery_LambdaVsAlbedo_plot_espresso_hr_51_Peg_b_4days_A_g-0.2}.png}
	\caption{51 Peg b; $A_g$ = 0.1; $\chi^2 = 0.56$}
\end{subfigure}


==> figures/tex_figure_espresso_hr_51_Peg_b_4days_HJ_aerosols_x1.tex <==
\begin{subfigure}[t]{0.5\hsize}
	\includegraphics[width=\hsize]{./figures/recovery_LambdaVsAlbedo_plot_espresso_hr_51_Peg_b_4days_HJ_aerosols_x1.png}
	\caption{51 Peg b; Model A ($\times 1$); $\chi^2 = 1.71$}
\end{subfigure}


==> figures/tex_figure_espresso_hr_51_Peg_b_4days_HJ_aerosols_x100.tex <==
\begin{subfigure}[t]{0.5\hsize}
	\includegraphics[width=\hsize]{./figures/recovery_LambdaVsAlbedo_plot_espresso_hr_51_Peg_b_4days_HJ_aerosols_x100.png}
	\caption{51 Peg b; Model A ($\times 100$); $\chi^2 = 4.37$}
\end{subfigure}


==> figures/tex_figure_espresso_hr_HD_209458_b_4days_A_g-0.2.tex <==
\begin{subfigure}[t]{0.5\hsize}
	\includegraphics[width=\hsize]{./figures/{recovery_LambdaVsAlbedo_plot_espresso_hr_HD_209458_b_4days_A_g-0.2}.png}
	\caption{HD 209458 b; $A_g$ = 0.1; $\chi^2 = 0.34$}
\end{subfigure}


==> figures/tex_figure_espresso_hr_HD_209458_b_4days_HJ_LowAlk_aerosols_x1.tex <==
\begin{subfigure}[t]{0.5\hsize}
	\includegraphics[width=\hsize]{./figures/recovery_LambdaVsAlbedo_plot_espresso_hr_HD_209458_b_4days_HJ_LowAlk_aerosols_x1.png}
	\caption{HD 209458 b; Model B ($\times 1$); $\chi^2 = 1.78$}
\end{subfigure}


==> figures/tex_figure_espresso_hr_HD_209458_b_4days_HJ_LowAlk_aerosols_x100.tex <==
\begin{subfigure}[t]{0.5\hsize}
	\includegraphics[width=\hsize]{./figures/recovery_LambdaVsAlbedo_plot_espresso_hr_HD_209458_b_4days_HJ_LowAlk_aerosols_x100.png}
	\caption{HD 209458 b; Model B ($\times 100$); $\chi^2 = 3.62$}
\end{subfigure}


==> figures/tex_figure_espresso_mhr_2ut_51_Peg_b_4days_A_g-0.2.tex <==
\begin{subfigure}[t]{0.5\hsize}
	\includegraphics[width=\hsize]{./figures/{recovery_LambdaVsAlbedo_plot_espresso_mhr_2ut_51_Peg_b_4days_A_g-0.2}.png}
	\caption{51 Peg b; $A_g$ = 0.1; $\chi^2 = 0.89$}
\end{subfigure}


==> figures/tex_figure_espresso_mhr_2ut_51_Peg_b_4days_HJ_aerosols_x1.tex <==
\begin{subfigure}[t]{0.5\hsize}
	\includegraphics[width=\hsize]{./figures/recovery_LambdaVsAlbedo_plot_espresso_mhr_2ut_51_Peg_b_4days_HJ_aerosols_x1.png}
	\caption{51 Peg b; Model A ($\times 1$); $\chi^2 = 3.45$}
\end{subfigure}


==> figures/tex_figure_espresso_mhr_2ut_51_Peg_b_4days_HJ_aerosols_x100.tex <==
\begin{subfigure}[t]{0.5\hsize}
	\includegraphics[width=\hsize]{./figures/recovery_LambdaVsAlbedo_plot_espresso_mhr_2ut_51_Peg_b_4days_HJ_aerosols_x100.png}
	\caption{51 Peg b; Model A ($\times 100$); $\chi^2 = 6.75$}
\end{subfigure}


==> figures/tex_figure_espresso_mhr_2ut_HD_209458_b_4days_A_g-0.2.tex <==
\begin{subfigure}[t]{0.5\hsize}
	\includegraphics[width=\hsize]{./figures/{recovery_LambdaVsAlbedo_plot_espresso_mhr_2ut_HD_209458_b_4days_A_g-0.2}.png}
	\caption{HD 209458 b; $A_g$ = 0.1; $\chi^2 = 0.54$}
\end{subfigure}


==> figures/tex_figure_espresso_mhr_2ut_HD_209458_b_4days_HJ_LowAlk_aerosols_x1.tex <==
\begin{subfigure}[t]{0.5\hsize}
	\includegraphics[width=\hsize]{./figures/recovery_LambdaVsAlbedo_plot_espresso_mhr_2ut_HD_209458_b_4days_HJ_LowAlk_aerosols_x1.png}
	\caption{HD 209458 b; Model B ($\times 1$); $\chi^2 = 3.44$}
\end{subfigure}


==> figures/tex_figure_espresso_mhr_2ut_HD_209458_b_4days_HJ_LowAlk_aerosols_x100.tex <==
\begin{subfigure}[t]{0.5\hsize}
	\includegraphics[width=\hsize]{./figures/recovery_LambdaVsAlbedo_plot_espresso_mhr_2ut_HD_209458_b_4days_HJ_LowAlk_aerosols_x100.png}
	\caption{HD 209458 b; Model B ($\times 100$); $\chi^2 = 6.68$}
\end{subfigure}


==> figures/tex_figure_espresso_mhr_4ut_51_Peg_b_4days_A_g-0.2.tex <==
\begin{subfigure}[t]{0.5\hsize}
	\includegraphics[width=\hsize]{./figures/{recovery_LambdaVsAlbedo_plot_espresso_mhr_4ut_51_Peg_b_4days_A_g-0.2}.png}
	\caption{51 Peg b; $A_g$ = 0.1; $\chi^2 = 1.91$}
\end{subfigure}


==> figures/tex_figure_espresso_mhr_4ut_51_Peg_b_4days_HJ_aerosols_x1.tex <==
\begin{subfigure}[t]{0.5\hsize}
	\includegraphics[width=\hsize]{./figures/recovery_LambdaVsAlbedo_plot_espresso_mhr_4ut_51_Peg_b_4days_HJ_aerosols_x1.png}
	\caption{51 Peg b; Model A ($\times 1$); $\chi^2 = 8.11$}
\end{subfigure}


==> figures/tex_figure_espresso_mhr_4ut_51_Peg_b_4days_HJ_aerosols_x100.tex <==
\begin{subfigure}[t]{0.5\hsize}
	\includegraphics[width=\hsize]{./figures/recovery_LambdaVsAlbedo_plot_espresso_mhr_4ut_51_Peg_b_4days_HJ_aerosols_x100.png}
	\caption{51 Peg b; Model A ($\times 100$); $\chi^2 = 14.87$}
\end{subfigure}


==> figures/tex_figure_espresso_mhr_4ut_HD_209458_b_4days_A_g-0.2.tex <==
\begin{subfigure}[t]{0.5\hsize}
	\includegraphics[width=\hsize]{./figures/{recovery_LambdaVsAlbedo_plot_espresso_mhr_4ut_HD_209458_b_4days_A_g-0.2}.png}
	\caption{HD 209458 b; $A_g$ = 0.1; $\chi^2 = 1.42$}
\end{subfigure}


==> figures/tex_figure_espresso_mhr_4ut_HD_209458_b_4days_HJ_LowAlk_aerosols_x1.tex <==
\begin{subfigure}[t]{0.5\hsize}
	\includegraphics[width=\hsize]{./figures/recovery_LambdaVsAlbedo_plot_espresso_mhr_4ut_HD_209458_b_4days_HJ_LowAlk_aerosols_x1.png}
	\caption{HD 209458 b; Model B ($\times 1$); $\chi^2 = 5.98$}
\end{subfigure}


==> figures/tex_figure_espresso_mhr_4ut_HD_209458_b_4days_HJ_LowAlk_aerosols_x100.tex <==
\begin{subfigure}[t]{0.5\hsize}
	\includegraphics[width=\hsize]{./figures/recovery_LambdaVsAlbedo_plot_espresso_mhr_4ut_HD_209458_b_4days_HJ_LowAlk_aerosols_x100.png}
	\caption{HD 209458 b; Model B ($\times 100$); $\chi^2 = 13.79$}
\end{subfigure}


==> figures/tex_figure_espresso_mhr_51_Peg_b_4days_A_g-0.2.tex <==
\begin{subfigure}[t]{0.5\hsize}
	\includegraphics[width=\hsize]{./figures/{recovery_LambdaVsAlbedo_plot_espresso_mhr_51_Peg_b_4days_A_g-0.2}.png}
	\caption{51 Peg b; $A_g$ = 0.1; $\chi^2 = 0.59$}
\end{subfigure}


==> figures/tex_figure_espresso_mhr_51_Peg_b_4days_HJ_aerosols_x1.tex <==
\begin{subfigure}[t]{0.5\hsize}
	\includegraphics[width=\hsize]{./figures/recovery_LambdaVsAlbedo_plot_espresso_mhr_51_Peg_b_4days_HJ_aerosols_x1.png}
	\caption{51 Peg b; Model A ($\times 1$); $\chi^2 = 1.94$}
\end{subfigure}


==> figures/tex_figure_espresso_mhr_51_Peg_b_4days_HJ_aerosols_x100.tex <==
\begin{subfigure}[t]{0.5\hsize}
	\includegraphics[width=\hsize]{./figures/recovery_LambdaVsAlbedo_plot_espresso_mhr_51_Peg_b_4days_HJ_aerosols_x100.png}
	\caption{51 Peg b; Model A ($\times 100$); $\chi^2 = 3.97$}
\end{subfigure}


==> figures/tex_figure_espresso_mhr_HD_209458_b_4days_A_g-0.2.tex <==
\begin{subfigure}[t]{0.5\hsize}
	\includegraphics[width=\hsize]{./figures/{recovery_LambdaVsAlbedo_plot_espresso_mhr_HD_209458_b_4days_A_g-0.2}.png}
	\caption{HD 209458 b; $A_g$ = 0.1; $\chi^2 = 0.29$}
\end{subfigure}


==> figures/tex_figure_espresso_mhr_HD_209458_b_4days_HJ_LowAlk_aerosols_x1.tex <==
\begin{subfigure}[t]{0.5\hsize}
	\includegraphics[width=\hsize]{./figures/recovery_LambdaVsAlbedo_plot_espresso_mhr_HD_209458_b_4days_HJ_LowAlk_aerosols_x1.png}
	\caption{HD 209458 b; Model B ($\times 1$); $\chi^2 = 1.72$}
\end{subfigure}


==> figures/tex_figure_espresso_mhr_HD_209458_b_4days_HJ_LowAlk_aerosols_x100.tex <==
\begin{subfigure}[t]{0.5\hsize}
	\includegraphics[width=\hsize]{./figures/recovery_LambdaVsAlbedo_plot_espresso_mhr_HD_209458_b_4days_HJ_LowAlk_aerosols_x100.png}
	\caption{HD 209458 b; Model B ($\times 100$); $\chi^2 = 3.51$}
\end{subfigure}


==> figures/tex_figure_espresso_uhr_51_Peg_b_4days_A_g-0.2.tex <==
\begin{subfigure}[t]{0.5\hsize}
	\includegraphics[width=\hsize]{./figures/{recovery_LambdaVsAlbedo_plot_espresso_uhr_51_Peg_b_4days_A_g-0.2}.png}
	\caption{51 Peg b; $A_g$ = 0.1; $\chi^2 = 0.73$}
\end{subfigure}


==> figures/tex_figure_espresso_uhr_51_Peg_b_4days_HJ_aerosols_x1.tex <==
\begin{subfigure}[t]{0.5\hsize}
	\includegraphics[width=\hsize]{./figures/recovery_LambdaVsAlbedo_plot_espresso_uhr_51_Peg_b_4days_HJ_aerosols_x1.png}
	\caption{51 Peg b; Model A ($\times 1$); $\chi^2 = 1.61$}
\end{subfigure}


==> figures/tex_figure_espresso_uhr_51_Peg_b_4days_HJ_aerosols_x100.tex <==
\begin{subfigure}[t]{0.5\hsize}
	\includegraphics[width=\hsize]{./figures/recovery_LambdaVsAlbedo_plot_espresso_uhr_51_Peg_b_4days_HJ_aerosols_x100.png}
	\caption{51 Peg b; Model A ($\times 100$); $\chi^2 = 3.6$}
\end{subfigure}


==> figures/tex_figure_espresso_uhr_HD_209458_b_4days_A_g-0.2.tex <==
\begin{subfigure}[t]{0.5\hsize}
	\includegraphics[width=\hsize]{./figures/{recovery_LambdaVsAlbedo_plot_espresso_uhr_HD_209458_b_4days_A_g-0.2}.png}
	\caption{HD 209458 b; $A_g$ = 0.1; $\chi^2 = 0.41$}
\end{subfigure}


==> figures/tex_figure_espresso_uhr_HD_209458_b_4days_HJ_LowAlk_aerosols_x1.tex <==
\begin{subfigure}[t]{0.5\hsize}
	\includegraphics[width=\hsize]{./figures/recovery_LambdaVsAlbedo_plot_espresso_uhr_HD_209458_b_4days_HJ_LowAlk_aerosols_x1.png}
	\caption{HD 209458 b; Model B ($\times 1$); $\chi^2 = 1.99$}
\end{subfigure}


==> figures/tex_figure_espresso_uhr_HD_209458_b_4days_HJ_LowAlk_aerosols_x100.tex <==
\begin{subfigure}[t]{0.5\hsize}
	\includegraphics[width=\hsize]{./figures/recovery_LambdaVsAlbedo_plot_espresso_uhr_HD_209458_b_4days_HJ_LowAlk_aerosols_x100.png}
	\caption{HD 209458 b; Model B ($\times 100$); $\chi^2 = 3.96$}
\end{subfigure}


==> figures/tex_figure_hires_51_Peg_b_4days_A_g-0.2.tex <==
\begin{subfigure}[t]{0.5\hsize}
	\includegraphics[width=\hsize]{./figures/{recovery_LambdaVsAlbedo_plot_hires_51_Peg_b_4days_A_g-0.2}.png}
	\caption{51 Peg b; $A_g$ = 0.1; $\chi^2 = 5.38$}
\end{subfigure}


==> figures/tex_figure_hires_51_Peg_b_4days_HJ_aerosols_x1.tex <==
\begin{subfigure}[t]{0.5\hsize}
	\includegraphics[width=\hsize]{./figures/recovery_LambdaVsAlbedo_plot_hires_51_Peg_b_4days_HJ_aerosols_x1.png}
	\caption{51 Peg b; Model A ($\times 1$); $\chi^2 = 7.84$}
\end{subfigure}


==> figures/tex_figure_hires_51_Peg_b_4days_HJ_aerosols_x100.tex <==
\begin{subfigure}[t]{0.5\hsize}
	\includegraphics[width=\hsize]{./figures/recovery_LambdaVsAlbedo_plot_hires_51_Peg_b_4days_HJ_aerosols_x100.png}
	\caption{51 Peg b; Model A ($\times 100$); $\chi^2 = 19.77$}
\end{subfigure}


==> figures/tex_figure_hires_55_Cnc_e_1days_A_g-0.2.tex <==
\begin{subfigure}[t]{0.5\hsize}
	\includegraphics[width=\hsize]{./figures/{recovery_LambdaVsAlbedo_plot_hires_55_Cnc_e_1days_A_g-0.2}.png}
	\caption{55 Cnc e; $A_g$ = 0.1; $\chi^2 = 0.67$}
\end{subfigure}


==> figures/tex_figure_hires_HD_109749_b_5days_A_g-0.2.tex <==
\begin{subfigure}[t]{0.5\hsize}
	\includegraphics[width=\hsize]{./figures/{recovery_LambdaVsAlbedo_plot_hires_HD_109749_b_5days_A_g-0.2}.png}
	\caption{HD 109749 b; $A_g$ = 0.1; $\chi^2 = 1.05$}
\end{subfigure}


==> figures/tex_figure_hires_HD_109749_b_5days_HJ_LowAlk_aerosols_x100.tex <==
\begin{subfigure}[t]{0.5\hsize}
	\includegraphics[width=\hsize]{./figures/recovery_LambdaVsAlbedo_plot_hires_HD_109749_b_5days_HJ_LowAlk_aerosols_x100.png}
	\caption{HD 109749 b; Model B ($\times 100$); $\chi^2 = 10.29$}
\end{subfigure}


==> figures/tex_figure_hires_HD_109749_b_5days_HJ_aerosols_x100.tex <==
\begin{subfigure}[t]{0.5\hsize}
	\includegraphics[width=\hsize]{./figures/recovery_LambdaVsAlbedo_plot_hires_HD_109749_b_5days_HJ_aerosols_x100.png}
	\caption{HD 109749 b; Model A ($\times 100$); $\chi^2 = 8.24$}
\end{subfigure}


==> figures/tex_figure_hires_HD_209458_b_4days_A_g-0.2.tex <==
\begin{subfigure}[t]{0.5\hsize}
	\includegraphics[width=\hsize]{./figures/{recovery_LambdaVsAlbedo_plot_hires_HD_209458_b_4days_A_g-0.2}.png}
	\caption{HD 209458 b; $A_g$ = 0.1; $\chi^2 = 2.04$}
\end{subfigure}


==> figures/tex_figure_hires_HD_209458_b_4days_HJ_LowAlk_aerosols_x1.tex <==
\begin{subfigure}[t]{0.5\hsize}
	\includegraphics[width=\hsize]{./figures/recovery_LambdaVsAlbedo_plot_hires_HD_209458_b_4days_HJ_LowAlk_aerosols_x1.png}
	\caption{HD 209458 b; Model B ($\times 1$); $\chi^2 = 8.17$}
\end{subfigure}


==> figures/tex_figure_hires_HD_209458_b_4days_HJ_LowAlk_aerosols_x100.tex <==
\begin{subfigure}[t]{0.5\hsize}
	\includegraphics[width=\hsize]{./figures/recovery_LambdaVsAlbedo_plot_hires_HD_209458_b_4days_HJ_LowAlk_aerosols_x100.png}
	\caption{HD 209458 b; Model B ($\times 100$); $\chi^2 = 15.94$}
\end{subfigure}


==> figures/tex_figure_hires_HD_76700_b_4days_A_g-0.2.tex <==
\begin{subfigure}[t]{0.5\hsize}
	\includegraphics[width=\hsize]{./figures/{recovery_LambdaVsAlbedo_plot_hires_HD_76700_b_4days_A_g-0.2}.png}
	\caption{HD 76700 b; $A_g$ = 0.1; $\chi^2 = 2.13$}
\end{subfigure}


==> figures/tex_figure_hires_HD_76700_b_4days_HJ_LowAlk_aerosols_x1.tex <==
\begin{subfigure}[t]{0.5\hsize}
	\includegraphics[width=\hsize]{./figures/recovery_LambdaVsAlbedo_plot_hires_HD_76700_b_4days_HJ_LowAlk_aerosols_x1.png}
	\caption{HD 76700 b; Model B ($\times 1$); $\chi^2 = 10.91$}
\end{subfigure}


==> figures/tex_figure_hires_HD_76700_b_4days_HJ_aerosols_x1.tex <==
\begin{subfigure}[t]{0.5\hsize}
	\includegraphics[width=\hsize]{./figures/recovery_LambdaVsAlbedo_plot_hires_HD_76700_b_4days_HJ_aerosols_x1.png}
	\caption{HD 76700 b; Model A ($\times 1$); $\chi^2 = 3.0$}
\end{subfigure}


==> figures/tex_figure_resolution_espresso_hr_51_Peg_b_4days_A_g-0.2.tex <==
\begin{subfigure}[t]{0.5\hsize}
	\includegraphics[width=\hsize]{./figures/{recovery_LambdaVsAlbedo_plot_resolution_espresso_hr_51_Peg_b_4days_A_g-0.2}.png}
	\caption{51 Peg b; $A_g$ = 0.1; $\chi^2 = 12.59$}
\end{subfigure}


==> figures/tex_figure_resolution_espresso_hr_HD_209458_b_4days_A_g-0.2.tex <==
\begin{subfigure}[t]{0.5\hsize}
	\includegraphics[width=\hsize]{./figures/{recovery_LambdaVsAlbedo_plot_resolution_espresso_hr_HD_209458_b_4days_A_g-0.2}.png}
	\caption{HD 209458 b; $A_g$ = 0.1; $\chi^2 = 1.41$}
\end{subfigure}


==> figures/tex_figure_resolution_espresso_mhr_2ut_51_Peg_b_4days_A_g-0.2.tex <==
\begin{subfigure}[t]{0.5\hsize}
	\includegraphics[width=\hsize]{./figures/{recovery_LambdaVsAlbedo_plot_resolution_espresso_mhr_2ut_51_Peg_b_4days_A_g-0.2}.png}
	\caption{51 Peg b; $A_g$ = 0.1; $\chi^2 = 19.87$}
\end{subfigure}


==> figures/tex_figure_resolution_espresso_mhr_2ut_HD_209458_b_4days_A_g-0.2.tex <==
\begin{subfigure}[t]{0.5\hsize}
	\includegraphics[width=\hsize]{./figures/{recovery_LambdaVsAlbedo_plot_resolution_espresso_mhr_2ut_HD_209458_b_4days_A_g-0.2}.png}
	\caption{HD 209458 b; $A_g$ = 0.1; $\chi^2 = 2.83$}
\end{subfigure}


==> figures/tex_figure_resolution_espresso_mhr_4ut_51_Peg_b_4days_A_g-0.2.tex <==
\begin{subfigure}[t]{0.5\hsize}
	\includegraphics[width=\hsize]{./figures/{recovery_LambdaVsAlbedo_plot_resolution_espresso_mhr_4ut_51_Peg_b_4days_A_g-0.2}.png}
	\caption{51 Peg b; $A_g$ = 0.1; $\chi^2 = 25.82$}
\end{subfigure}


==> figures/tex_figure_resolution_espresso_mhr_4ut_HD_209458_b_4days_A_g-0.2.tex <==
\begin{subfigure}[t]{0.5\hsize}
	\includegraphics[width=\hsize]{./figures/{recovery_LambdaVsAlbedo_plot_resolution_espresso_mhr_4ut_HD_209458_b_4days_A_g-0.2}.png}
	\caption{HD 209458 b; $A_g$ = 0.1; $\chi^2 = 5.18$}
\end{subfigure}


==> figures/tex_figure_resolution_espresso_mhr_51_Peg_b_4days_A_g-0.2.tex <==
\begin{subfigure}[t]{0.5\hsize}
	\includegraphics[width=\hsize]{./figures/{recovery_LambdaVsAlbedo_plot_resolution_espresso_mhr_51_Peg_b_4days_A_g-0.2}.png}
	\caption{51 Peg b; $A_g$ = 0.1; $\chi^2 = 17.49$}
\end{subfigure}


==> figures/tex_figure_resolution_espresso_mhr_HD_209458_b_4days_A_g-0.2.tex <==
\begin{subfigure}[t]{0.5\hsize}
	\includegraphics[width=\hsize]{./figures/{recovery_LambdaVsAlbedo_plot_resolution_espresso_mhr_HD_209458_b_4days_A_g-0.2}.png}
	\caption{HD 209458 b; $A_g$ = 0.1; $\chi^2 = 1.74$}
\end{subfigure}


==> figures/tex_figure_resolution_espresso_uhr_51_Peg_b_4days_A_g-0.2.tex <==
\begin{subfigure}[t]{0.5\hsize}
	\includegraphics[width=\hsize]{./figures/{recovery_LambdaVsAlbedo_plot_resolution_espresso_uhr_51_Peg_b_4days_A_g-0.2}.png}
	\caption{51 Peg b; $A_g$ = 0.1; $\chi^2 = 7.62$}
\end{subfigure}


==> figures/tex_figure_resolution_espresso_uhr_HD_209458_b_4days_A_g-0.2.tex <==
\begin{subfigure}[t]{0.5\hsize}
	\includegraphics[width=\hsize]{./figures/{recovery_LambdaVsAlbedo_plot_resolution_espresso_uhr_HD_209458_b_4days_A_g-0.2}.png}
	\caption{HD 209458 b; $A_g$ = 0.1; $\chi^2 = 0.51$}
\end{subfigure}


==> recovery_figures_.tex <==
\begin{figure*}
	\caption{Recovered albedos with ESPRESSO (MHR mode)}
	\label{fig:espresso_mhr}
	\end{figure*}\begin{figure*}
	\caption{Recovered albedos with ESPRESSO (HR mode)}
	\label{fig:espresso_hr}
	\begin{subfigure}[t]{0.5\hsize}
		\includegraphics[width=\hsize]{./figures/recovery_LambdaVsAlbedo_plot_espresso_hr_51_Peg_b_4days_HJ_aerosols_x100.png}
		\caption{51 Peg b; Model A ($\times 100$); $\chi^2 = 12.13$}
	\end{subfigure}
	\end{figure*}\begin{figure*}
	\caption{Recovered albedos with ESPRESSO (UHR mode)}
	\label{fig:espresso_uhr}
	\end{figure*}\begin{figure*}
	\caption{Recovered albedos with HIRES}
	\label{fig:hires}
	\end{figure*}

==> recovery_figures_espresso.tex <==
\begin{figure*}
	\caption{Recovered albedos with ESPRESSO (MHR mode)}
	\label{fig:espresso_mhr}
	\begin{subfigure}[t]{0.5\hsize}
		\includegraphics[width=\hsize]{./figures/{recovery_LambdaVsAlbedo_plot_espresso_mhr_51_Peg_b_4days_A_g-0.1}.png}
		\caption{51 Peg b; $A_g$ = 1.00; $\chi^2 = 0.42$}
	\end{subfigure}
	\begin{subfigure}[t]{0.5\hsize}
		\includegraphics[width=\hsize]{./figures/recovery_LambdaVsAlbedo_plot_espresso_mhr_51_Peg_b_4days_HJ_aerosols_x100.png}
		\caption{51 Peg b; Model A ($\times 100$); $\chi^2 = 19.67$}
	\end{subfigure}
	
\begin{subfigure}[t]{0.5\hsize}
		\includegraphics[width=\hsize]{./figures/recovery_LambdaVsAlbedo_plot_espresso_mhr_51_Peg_b_4days_HJ_aerosols_x1.png}
		\caption{51 Peg b; Model A ($\times 1$); $\chi^2 = 9.87$}
	\end{subfigure}
	\begin{subfigure}[t]{0.5\hsize}
		\includegraphics[width=\hsize]{./figures/{recovery_LambdaVsAlbedo_plot_espresso_mhr_HD_209458_b_4days_A_g-0.1}.png}
		\caption{HD 209458 b; $A_g$ = 1.00; $\chi^2 = 0.03$}
	\end{subfigure}
	
\begin{subfigure}[t]{0.5\hsize}
		\includegraphics[width=\hsize]{./figures/recovery_LambdaVsAlbedo_plot_espresso_mhr_HD_209458_b_4days_HJ_LowAlk_aerosols_x100.png}
		\caption{HD 209458 b; Model B ($\times 100$); $\chi^2 = 8.45$}
	\end{subfigure}
	\begin{subfigure}[t]{0.5\hsize}
		\includegraphics[width=\hsize]{./figures/recovery_LambdaVsAlbedo_plot_espresso_mhr_HD_209458_b_4days_HJ_LowAlk_aerosols_x1.png}
		\caption{HD 209458 b; Model B ($\times 1$); $\chi^2 = 5.41$}
	\end{subfigure}
	
\end{figure*}\begin{figure*}
	\caption{Recovered albedos with ESPRESSO (HR mode)}
	\label{fig:espresso_hr}
	\begin{subfigure}[t]{0.5\hsize}
		\includegraphics[width=\hsize]{./figures/{recovery_LambdaVsAlbedo_plot_espresso_hr_51_Peg_b_4days_A_g-0.1}.png}
		\caption{51 Peg b; $A_g$ = 1.00; $\chi^2 = 0.15$}
	\end{subfigure}
	\begin{subfigure}[t]{0.5\hsize}
		\includegraphics[width=\hsize]{./figures/recovery_LambdaVsAlbedo_plot_espresso_hr_51_Peg_b_4days_HJ_aerosols_x100.png}
		\caption{51 Peg b; Model A ($\times 100$); $\chi^2 = 14.26$}
	\end{subfigure}
	
\begin{subfigure}[t]{0.5\hsize}
		\includegraphics[width=\hsize]{./figures/recovery_LambdaVsAlbedo_plot_espresso_hr_51_Peg_b_4days_HJ_aerosols_x1.png}
		\caption{51 Peg b; Model A ($\times 1$); $\chi^2 = 9.09$}
	\end{subfigure}
	\begin{subfigure}[t]{0.5\hsize}
		\includegraphics[width=\hsize]{./figures/{recovery_LambdaVsAlbedo_plot_espresso_hr_HD_209458_b_4days_A_g-0.1}.png}
		\caption{HD 209458 b; $A_g$ = 1.00; $\chi^2 = 0.03$}
	\end{subfigure}
	
\begin{subfigure}[t]{0.5\hsize}
		\includegraphics[width=\hsize]{./figures/recovery_LambdaVsAlbedo_plot_espresso_hr_HD_209458_b_4days_HJ_LowAlk_aerosols_x100.png}
		\caption{HD 209458 b; Model B ($\times 100$); $\chi^2 = 7.33$}
	\end{subfigure}
	\begin{subfigure}[t]{0.5\hsize}
		\includegraphics[width=\hsize]{./figures/recovery_LambdaVsAlbedo_plot_espresso_hr_HD_209458_b_4days_HJ_LowAlk_aerosols_x1.png}
		\caption{HD 209458 b; Model B ($\times 1$); $\chi^2 = 5.58$}
	\end{subfigure}
	
\end{figure*}\begin{figure*}
	\caption{Recovered albedos with ESPRESSO (UHR mode)}
	\label{fig:espresso_uhr}
	\begin{subfigure}[t]{0.5\hsize}
		\includegraphics[width=\hsize]{./figures/{recovery_LambdaVsAlbedo_plot_espresso_uhr_51_Peg_b_4days_A_g-0.1}.png}
		\caption{51 Peg b; $A_g$ = 1.00; $\chi^2 = 0.12$}
	\end{subfigure}
	\begin{subfigure}[t]{0.5\hsize}
		\includegraphics[width=\hsize]{./figures/recovery_LambdaVsAlbedo_plot_espresso_uhr_51_Peg_b_4days_HJ_aerosols_x100.png}
		\caption{51 Peg b; Model A ($\times 100$); $\chi^2 = 7.07$}
	\end{subfigure}
	
\begin{subfigure}[t]{0.5\hsize}
		\includegraphics[width=\hsize]{./figures/recovery_LambdaVsAlbedo_plot_espresso_uhr_51_Peg_b_4days_HJ_aerosols_x1.png}
		\caption{51 Peg b; Model A ($\times 1$); $\chi^2 = 4.88$}
	\end{subfigure}
	\begin{subfigure}[t]{0.5\hsize}
		\includegraphics[width=\hsize]{./figures/{recovery_LambdaVsAlbedo_plot_espresso_uhr_HD_209458_b_4days_A_g-0.1}.png}
		\caption{HD 209458 b; $A_g$ = 1.00; $\chi^2 = 0.03$}
	\end{subfigure}
	
\begin{subfigure}[t]{0.5\hsize}
		\includegraphics[width=\hsize]{./figures/recovery_LambdaVsAlbedo_plot_espresso_uhr_HD_209458_b_4days_HJ_LowAlk_aerosols_x100.png}
		\caption{HD 209458 b; Model B ($\times 100$); $\chi^2 = 3.79$}
	\end{subfigure}
	\begin{subfigure}[t]{0.5\hsize}
		\includegraphics[width=\hsize]{./figures/recovery_LambdaVsAlbedo_plot_espresso_uhr_HD_209458_b_4days_HJ_LowAlk_aerosols_x1.png}
		\caption{HD 209458 b; Model B ($\times 1$); $\chi^2 = 1.98$}
	\end{subfigure}
	
\end{figure*}\begin{figure*}
	\caption{Recovered albedos with HIRES}
	\label{fig:hires}
	\end{figure*}

==> recovery_figures_hires.tex <==
\begin{figure*}
	\caption{Recovered albedos with ESPRESSO (MHR mode)}
	\label{fig:espresso_mhr}
	\end{figure*}\begin{figure*}
	\caption{Recovered albedos with ESPRESSO (HR mode)}
	\label{fig:espresso_hr}
	\end{figure*}\begin{figure*}
	\caption{Recovered albedos with ESPRESSO (UHR mode)}
	\label{fig:espresso_uhr}
	\end{figure*}\begin{figure*}
	\caption{Recovered albedos with HIRES}
	\label{fig:hires}
	\begin{subfigure}[t]{0.5\hsize}
		\includegraphics[width=\hsize]{./figures/{recovery_LambdaVsAlbedo_plot_hires_51_Peg_b_4days_A_g-0.1}.png}
		\caption{51 Peg b; $A_g$ = 0.48; $\chi^2 = 0.47$}
	\end{subfigure}
	\begin{subfigure}[t]{0.5\hsize}
		\includegraphics[width=\hsize]{./figures/recovery_LambdaVsAlbedo_plot_hires_51_Peg_b_4days_HJ_aerosols_x100.png}
		\caption{51 Peg b; Model A ($\times 100$); $\chi^2 = 19.80$}
	\end{subfigure}
	
\begin{subfigure}[t]{0.5\hsize}
		\includegraphics[width=\hsize]{./figures/recovery_LambdaVsAlbedo_plot_hires_51_Peg_b_4days_HJ_aerosols_x1.png}
		\caption{51 Peg b; Model A ($\times 1$); $\chi^2 = 10.05$}
	\end{subfigure}
	\begin{subfigure}[t]{0.5\hsize}
		\includegraphics[width=\hsize]{./figures/{recovery_LambdaVsAlbedo_plot_hires_55_Cnc_e_1days_A_g-0.1}.png}
		\caption{55 Cnc e; $A_g$ = 0.48; $\chi^2 = 0.89$}
	\end{subfigure}
	
\begin{subfigure}[t]{0.5\hsize}
		\includegraphics[width=\hsize]{./figures/{recovery_LambdaVsAlbedo_plot_hires_HD_109749_b_5days_A_g-0.1}.png}
		\caption{HD 109749 b; $A_g$ = 0.48; $\chi^2 = 0.16$}
	\end{subfigure}
	\begin{subfigure}[t]{0.5\hsize}
		\includegraphics[width=\hsize]{./figures/recovery_LambdaVsAlbedo_plot_hires_HD_109749_b_5days_HJ_aerosols_x100.png}
		\caption{HD 109749 b; Model A ($\times 100$); $\chi^2 = 14.48$}
	\end{subfigure}
	
\begin{subfigure}[t]{0.5\hsize}
		\includegraphics[width=\hsize]{./figures/recovery_LambdaVsAlbedo_plot_hires_HD_109749_b_5days_HJ_LowAlk_aerosols_x100.png}
		\caption{HD 109749 b; Model B ($\times 100$); $\chi^2 = 9.37$}
	\end{subfigure}
	\begin{subfigure}[t]{0.5\hsize}
		\includegraphics[width=\hsize]{./figures/{recovery_LambdaVsAlbedo_plot_hires_HD_209458_b_4days_A_g-0.1}.png}
		\caption{HD 209458 b; $A_g$ = 0.48; $\chi^2 = 0.48$}
	\end{subfigure}
	
\begin{subfigure}[t]{0.5\hsize}
		\includegraphics[width=\hsize]{./figures/recovery_LambdaVsAlbedo_plot_hires_HD_209458_b_4days_HJ_LowAlk_aerosols_x100.png}
		\caption{HD 209458 b; Model B ($\times 100$); $\chi^2 = 23.67$}
	\end{subfigure}
	\begin{subfigure}[t]{0.5\hsize}
		\includegraphics[width=\hsize]{./figures/recovery_LambdaVsAlbedo_plot_hires_HD_209458_b_4days_HJ_LowAlk_aerosols_x1.png}
		\caption{HD 209458 b; Model B ($\times 1$); $\chi^2 = 15.17$}
	\end{subfigure}
	
\begin{subfigure}[t]{0.5\hsize}
		\includegraphics[width=\hsize]{./figures/{recovery_LambdaVsAlbedo_plot_hires_HD_76700_b_4days_A_g-0.1}.png}
		\caption{HD 76700 b; $A_g$ = 0.48; $\chi^2 = 0.27$}
	\end{subfigure}
	\begin{subfigure}[t]{0.5\hsize}
		\includegraphics[width=\hsize]{./figures/recovery_LambdaVsAlbedo_plot_hires_HD_76700_b_4days_HJ_aerosols_x1.png}
		\caption{HD 76700 b; Model A ($\times 1$); $\chi^2 = 5.36$}
	\end{subfigure}
	
\begin{subfigure}[t]{0.5\hsize}
		\includegraphics[width=\hsize]{./figures/recovery_LambdaVsAlbedo_plot_hires_HD_76700_b_4days_HJ_LowAlk_aerosols_x1.png}
		\caption{HD 76700 b; Model B ($\times 1$); $\chi^2 = 2.46$}
	\end{subfigure}
	\end{figure*}
